The Power of Abstract MAC Layer: A Fault-tolerance Perspective

This paper studies the power of the "abstract MAC layer" model in a single-hop asynchronous network. The model captures primitive properties of modern wireless MAC protocols. In this model, Newport [PODC '14] proves that it is impossible to achieve deterministic consensus when nodes may crash. Subsequently, Newport and Robinson [DISC '18] present randomized consensus algorithms that terminate with O(n3 log n) expected broadcasts in a system of n nodes. We are not aware of any results on other fault-tolerant distributed tasks in this model. We first study the computability aspect of the abstract MAC layer. We present a wait-free algorithm that implements an atomic register. Furthermore, we show that in general, k-set consensus is impossible. Second, we aim to minimize storage complexity. Existing algorithms require {\Omega}(n log n) bits. We propose four wait-free consensus algorithms that only need constant storage complexity. (Two approximate consensus and two randomized binary consensus algorithms.) One randomized algorithm terminates with O(n log n) expected broadcasts. All our consensus algorithms are anonymous, meaning that at the algorithm level, nodes do not need to have a unique identifier.

==> MAC-RBC-2024.tex <==
\begin{algorithm*}
\caption{MAC-RBC Algorithm: Steps at each node $i$ with input $x_i$}
\label{alg:MAC-RBC}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
\item[] $seen_i[0]$ \Comment{(Boolean, phase), initialized to $(false, 0)$}
\item[] $seen_i[1]$ \Comment{(Boolean, phase), initialized to $(false, 0)$}
\item[] $seen_i^2[0]$ \Comment{(Boolean, phase), initialized to $(false, 0)$}
\item[] $seen_i^2[1]$ \Comment{(Boolean, phase), initialized to $(false, 0)$}
\item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
\item[] $p_i$ \Comment{phase, initialized to $0$}
\item[] $proposal_i$ \Comment{(value, phase), initialized to $(\perp,0)$}
\item[] $n'$ \Comment{estimated system size, initialized to $1$}
\item[] $knownIDs$ \Comment{set of known IDs, initialized to $\{i\}$}
\vspace{-5pt}
\item[] \hrulefill    
\vspace{-15pt}
\begin{multicols}{2}
    %\For{$p_i \gets 1 \dots$}
    \State $\texttt{mac-broadcast}(\texttt{ID}, i)$
    \While{true}
        \State $p_{old} \gets p_i$
        \State $\texttt{mac-broadcast}(\texttt{VALUE}, v_i, p_i)$
        %\State \texttt{lock()}
        %\If{$p_{next} = p_i$}
        
        % old PODC code
            % \If{$proposal_i.phase < p_i$}
                
            %     \State $\texttt{mac-broadcast}(\texttt{PROPOSAL}, v_i, p_i)$
        
            % \Else
            %     \State $(v_i, p_i) \gets proposal_i$
                
            % \EndIf
        % old PODC code    
            \If{$proposal_i.phase \geq p_i$}
                \State $(v_i, p_i) \gets proposal_i$
            \EndIf
            \State $\texttt{mac-broadcast}(\texttt{PROPOSAL}, v_i, p_i)$
            
            \If{$p_{old} \neq p_i$}
                \State \textbf{go to} line 2 in  $p_i$ \Comment{``Jump'' to $p_i$}
            \ElsIf{$seen_i[-v_i].phase < p_i$} 
                \State \textbf{output} $v_i$
            %\ElsIf{$seen_i[-v_i].phase = p_i$} 
                % \If{$seen_i[-v_i].value =$ false}
                %     \State \textbf{return} $v_i$
                % \EndIf
            \Else    %\Comment{Conciliation}
                %\State \textbf{go to} phase $p_i+1$ \Comment{``Move'' to $p_i+1$}
                \State \texttt{mac-broadcast}($\texttt{VALUE}^2, v_i, p_i$)
                \If{$seen_i^2[-v_i].phase > p_i$}
                    \State $(v_i, p_i) \gets seen_i^2[-v_i]$
                    \State \textbf{go to} line 2 in  $p_i$ \Comment{``Jump'' to $p_i$}
                \ElsIf{$seen_i^2[-v_i]=(true, p_i)$}
                %\ElsIf{$seen_i^2[-v_i].phase = p_i$}
                    %\If{$seen_i^2[-v_i]=(true, p_i)$}
                        \State $v_i \gets$\textsc{MAC-DoubleFirstMover($n'$)}
                    %\EndIf
                    %\State $p_i \gets p_i + 1$ \Comment{``Move'' to $p_i$}
                \EndIf    
                \State $p_i \gets p_i + 1$ \Comment{``Move'' to $p_i$}
            \EndIf
        %\EndIf
        %\State \texttt{unlock()}
    %\EndFor
    \EndWhile
    
    \columnbreak
    
    \item[$\slash\slash$ \textit{Background message handler}]
    \Upon{receive($\texttt{ID}, j$)} 
        \If{$j \in knownIDs$ \qinzi{$\notin$?}}
            \State \texttt{mac-broadcast}($\texttt{ID}, j$)
            \State $knownIDs \gets knownIDs \cup \{j\}$
            \State $n' \gets n' + 1$
        \EndIf    
    \EndUpon
    \item[]
    \Upon{receive($\texttt{VALUE}, v, p$)} 
        \If{$p \geq seen_i[v].phase$}
            \State $seen_i[v] \gets (true, p)$
        \EndIf    
        %\State \texttt{mac-broadcast}($\texttt{VALUE}, v$)
    \EndUpon
    \item[]
    \Upon{receive($\texttt{VALUE}^2, v, p$)} 
        \If{$p \geq seen_i^2[v].phase$}
            \State $seen_i^2[v] \gets (true, p)$
        \EndIf    
        %\State \texttt{mac-broadcast}($\texttt{VALUE}, v$)
    \EndUpon
    \item[]
    \Upon{receive($\texttt{PROPOSAL}, v, p$)} 
        \If{$p \geq proposal_i.phase$}
            \State $proposal_i \gets (v, p)$
        \EndIf
        %\State \texttt{mac-broadcast}($\texttt{PROPOSAL}, v$)
    \EndUpon
    % \Statex
    % \item[]
    % \item[]
\end{multicols}
\vspace{-10pt}
\end{algorithmic}
\end{algorithm*}

==> approximate.tex <==
\section{Practical Considerations}
\label{s:practical}

As we will show in Section \ref{s:prior}, using a retransmission-based mechanism to ensure a reliable channel \cite{AA_nancy,welch_book} incurs prohibitively high storage complexity. Our design does not rely on reliable delivery of all the messages. Instead, each node broadcasts its state value  periodically throughout the execution, and \textit{some} messages might never be delivered.  This design together with the property of fair lossy channels imply the following \textit{eventual progress property}:

\begin{assumption}[Eventual Progress]
    \label{as:eventual-progress}
    Given a broadcast interval $t$ (as specified in the algorithm), there exists a finite time bound $\Delta$ such that for each point of time $t_0$ and each fault-free node $i$, if node $i$ broadcasts some messages every $t$ units of time during the time interval $[t_0,t_0+\Delta]$, then every fault-free node (trivially including $i$ itself) will receive at least one message during $[t_0,t_0+\Delta]$.
\end{assumption}

Note that $\Delta$ is a parameter depending on $t$. For brevity, we omit $t$ in the notation. Our algorithms do not use $\Delta$, as it is an (environment) parameter that depends on how the underlying lossy channels behave, and generally unknown. We only use $\Delta$ in our convergence analysis. 

%\qinzi{Do we need to elaborate a little more about this assumptions?  Also, reviewer 1 says ``What if the scheduler chooses to fail a sender within any given period of Delta before it broadcasts the message enough times?'' I'm not sure if the scheduler refers to the adversary?}

%\lewis{Sure. How would you want to elaborate? Yes, scheduler = adversary. But since we do not consider crash-recovery now. We don't need to consider that case, i.e., we can ignore that comment.}

%In practical applications,  Assumption \ref{as:1} holds if node $i$ broadcasts periodically (e.g., every 100ms), instead of broadcasting messages infinitely many times.

The eventual progress assumption is intuitively similar to the \textit{eventual delivery} assumption of retransmission-based mechanism that emulates a reliable channel on top of a lossy channel \cite{AA_nancy,welch_book,Reliable-transmission_JACM1994} -- between any pair of fault-free nodes, \textit{any} message is  delivered in a bounded time. The subtle difference is that our eventual progress assumption only requires \textit{one} message to be delivered in the $\Delta$-time interval, not all messages, to be delivered. 

We illustrate the difference between different communication models and approaches in Figure \ref{f:model}. Figure \ref{fig:reliable} represents the reliable channel, in which all the messages are delivered. Figure \ref{fig:CR} represents the emulated reliable channel on top of lossy channels (e.g., using an RMTP protocol \cite{Reliable-transmission_JACM1994} or adopting TCP). Messages might be lost, but with enough retransmission, all the messages are guaranteed to be delivered. In the example, both $m_1$ and $m_2$ are delivered after two lost messages. Figure \ref{fig:CR-lossy} illustrates our approach in a lossy channel. We do not require delivery for all the messages; instead, we only need the delivery of some messages ($m_3$ and $m_6$ in the example).
In Figure \ref{fig:CR-lossy}, the maximum duration between two dashed lines are defined as $\Delta$ as per Assumption \ref{as:eventual-progress}. Our algorithms work correctly as long as one message in the interval is delivered, even if some of the messages are never delivered at the receiver. 

%As aforementioned, since we are interested in storage-optimal consensus algorithms, re-transmitting (potentially lost) messages to simulate a reliable channel with the eventual delivery property is not a feasible solution, as re-transmission requires unbounded space in the worst case \cite{Reliable-transmission_JACM1994}. 


\section{Approximate Consensus Algorithms}
\label{s:approximate}

\begin{figure*}[!ht]
	\begin{subfigure}[b]{0.32\textwidth}
	    \centering
		\begin{tikzpicture}
		    \draw[-latex, very thick] (0,0) -- (4,0);
		    \node (a) at (-0.6,0) {\small{node $i$}};
		    \draw[-latex, very thick] (0,-1) -- (4,-1);
		    \node (b) at (-0.6,-1) {\small{node $j$}};
		    
		  %  \draw[very thick, fill=white] (2.4,-0.75) rectangle (4,-1.25);
		  %  \node (c) at (3.2,-1) {\small{Crash}};
		  %  \filldraw[color=white] (3.9,-0.7) rectangle (4.1,-1.3);
		    
		  %  \draw[thick, color=red, -latex] (0.5,0) -- (2.8,-0.75);
		    \draw[thick, color=blue, -latex] (1,0) -- (2,-1);
		    \draw[thick, color=blue, -latex] (2,0) -- (3,-1);
		    \node (d) at (1,0.2) {\small{$m_1$}};
		    \node (3) at (2,0.2) {\small{$m_2$}};
		\end{tikzpicture}
		\caption{Reliable Channel}
		\label{fig:reliable}
	\end{subfigure}
	\hfill %%
	\begin{subfigure}[b]{0.32\textwidth}
		\begin{tikzpicture}
		    \draw[-latex, very thick] (0,0) -- (4,0);
		    \node (a) at (-0.6,0) {\small{node $i$}};
		    \draw[-latex, very thick] (0,-1) -- (4,-1);
		    \node (b) at (-0.6,-1) {\small{node $j$}};
		    
		    \draw[thick, color=red, -latex] (0.5,0) -- (0.8,-0.5);
		    \draw[thick, color=red, -latex] (1,0) -- (1.3,-0.5);
		    \draw[thick, color=blue, -latex] (1.5,0) -- (2.1,-1);
		    \draw [thick,decorate,decoration={brace,amplitude=3pt}] (0.5,0.1) -- (1.5,0.1) node [black,midway,yshift=8pt] {\small $m_1$};
		    
		    \draw[thick, color=red, -latex] (2,0) -- (2.3,-0.5);
		    \draw[thick, color=red, -latex] (2.5,0) -- (2.8,-0.5);
		    \draw[thick, color=blue, -latex] (3,0) -- (3.6,-1);
		    \draw [thick,decorate,decoration={brace,amplitude=3pt}] (2,0.1) -- (3,0.1) node [black,midway,yshift=8pt] {\small $m_2$};	    
		\end{tikzpicture}
		\caption{Emulated Reliable Channel}
		\label{fig:CR}
	\end{subfigure}  
	\hfill %%
	\begin{subfigure}[b]{0.32\textwidth}
		\begin{tikzpicture}
		    \draw[dashed, thick] (0.2,-1.25) -- (0.2,0.25);
		    \draw[dashed, thick] (2.9,-1.25) -- (2.9,0.25);
		
		    \draw[-latex, very thick] (0,0) -- (4,0);
		    \node (a) at (-0.6,0) {\small{node $i$}};
		    \draw[-latex, very thick] (0,-1) -- (4,-1);
		    \node (b) at (-0.6,-1) {\small{node $j$}};
		    
		    \draw[thick, color=red, -latex] (0.5,0) -- (0.8,-0.5);
		    \draw[thick, color=red, -latex] (1,0) -- (1.3,-0.5);
		    \draw[thick, color=blue, -latex] (1.5,0) -- (2.1,-1);
		    \node at (0.5,0.2) {\small{$m_1$}};
		    \node at (1,0.2) {\small{$m_2$}};
		    \node at (1.5,0.2) {\small{$m_3$}};
		    
		    \draw[thick, color=red, -latex] (2,0) -- (2.3,-0.5);
		    \draw[thick, color=red, -latex] (2.5,0) -- (2.8,-0.5);
		    \draw[thick, color=blue, -latex] (3.2,0) -- (3.8,-1);
		    \node at (2.0,0.2) {\small{$m_4$}};
		    \node at (2.5,0.2) {\small{$m_5$}};
		    \node at (3.2,0.2) {\small{$m_6$}};			    
		\end{tikzpicture}
		\caption{Our approach in Lossy Channel}
		\label{fig:CR-lossy}
	\end{subfigure}
	\caption{Illustration of different channel models. Thick black lines represent the timeline of nodes $i$ and $j$. Blue arrow represents that the message is delivered. Red arrow represents that the message is lost in the (underlying) lossy channel. The two dashed line in the rightmost figure represents the $\Delta$ defined in Assumption \ref{as:eventual-progress}.}
	\label{f:model}
\end{figure*}

	


\subsection{Why Prior Algorithms are not Practical?}
\label{s:prior}

Two major challenges of developing fault-tolerant algorithms for small connected devices are limited storage space and lossy links. These devices are designed to be cheap, power-efficient and small in size; hence, naturally, they are not equipped with large memory or disk. Moreover, they are usually built with low-end antenna(s), and communicate over wireless links. Message loss is common because of packet collisions, mobility, varying signal strength, obstacles in line-of-sight, etc. In 2013, a seminal study by USC \cite{WSN_loss_Sensys13} showed that around 35\% of the links are experiencing message loss higher than 50\% in a 60-node system deployed in indoor, outdoor, and multi-hop environments.
%https://people.eecs.berkeley.edu/~culler/cs294-f03/papers/zhao.pdf
 %Therefore, it is appropriate to model the communication as a lossy network. 

%Coordination under unreliable communication is known to be a huge challenge. The two generals problem \cite{Two-generals_SOSP1975} demonstrates that deterministic coordination is impossible with unreliable links. Plus, 

%Recall that we assume lossy links may duplicate, reorder and lose messages within a finite amount of time $\Delta$.
Theoretically speaking, lossy links that can duplicate, lose, reorder messages make the reliable message transmission problem (RMTP) impossible when a node has only a finite amount of storage space \cite{Reliable-transmission_JACM1994}. Intuitively, this is because \textit{a priori}, each node does not know how many times a message $m$ needs to be retransmitted so that $m$ will be reliably delivered at the receiver, i.e., $\Delta$ in Assumption \ref{as:eventual-progress} is unknown. Hence, the node needs to use a  sequence number (in the same vein of TCP) to distinguish messages. The size of the sequence number is proportional to the number of times that a message is retransmitted during the $\Delta$ time interval. Since such a sequence number is needed for every other node for solving RMTP, the total amount of storage required could easily blow up.

%Worse, this unavoidable overhead is only for emulating a single reliable link. To communicate with other $n-1$ nodes reliably, the overhead increases by $O(n)$ times.

%The impossibility result in \cite{Reliable-transmission_JACM1994} implies that any RMTP algorithm on top of lossy links that may reorder, lose, and duplicate messages requires to store all the information exchanged during the time interval $\Delta$.



From a practical perspective, it is typical to assume that TCP works reasonably well in the normal case with stable network connections (i.e., no malicious intruders or disastrous events). However, there are several known drawbacks of using TCP in connected things application, especially when networks may be lossy. First, TCP's header size is 3 to 7 times than UDP's header. Second, TCP is stateful, and needs to maintain buffers and other control data. Third, TCP needs to maintain and retry connection, if it is disrupted. In fact, there are several studies showing the limitations of using TCP in wireless networks (e.g., \cite{TCP_Wireless_study_2008,TCP_iot_2018}).

Prior approximate consensus algorithms are based on the assumption of reliable channels (e.g., \cite{AA_Fekete_aoptimal,AA_Dolev_1986,vaidya_PODC12,Tseng_general,Sundaram_condition,Sundaram_Control_Consensus_Allerton19,Panagou_Consensus_robotics,Panagou_Consensus_robotic2,Xavier_consensus_robotics,dynamic_agreement,dynamic_Byzantine,dynamic_consensus}). 
Due to the implication of  \cite{Reliable-transmission_JACM1994} and limitations of TCP-based implementations, these algorithms are not practical for small devices in lossy networks, because these devices are equipped with limited storage and not able to store all the necessary control information for using an RMTP protocol or TCP. 

Some recent algorithms in control systems \cite{Mehran_control_consensus_TAC18,Mehran_clock_consensus_TCNS18,Mehran_control_consensus_Automata17} adopt a slightly different design that tolerates partially synchronous networks where some messages might be lost. These algorithms work fine for most control systems that only require ``eventual convergence.'' In other words, each node does \textit{not} know the time when an approximate consensus, namely the $\epsilon$-agreement condition, has been achieved, and the algorithms only guarantee that at some \textit{unknown} point of time, the condition is satisfied. This eventual convergence property limits the applicability of their solutions. For example, if a swarm of robots need to learn the gathering location before making any movement, then our algorithms can be used, because of the termination property. Prior control algorithms \cite{Mehran_control_consensus_TAC18,Mehran_clock_consensus_TCNS18,Mehran_control_consensus_Automata17} do not naturally output any value, nor indicate the time when $\epsilon$-agreement is reached. Extra mechanisms need to be designed. Another drawback is that these algorithms do not tolerate message reordering without usage a potentially large sequence number.

\begin{algorithm}
\caption{AC Algorithm: Steps at each node $i$}
\label{alg:AC}
\begin{algorithmic}[1]
\item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
\item[] $p_i$ \Comment{phase, initialized to $0$}
\item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
\item[] \hrulefill    
\begin{multicols}{2}
    \For{$p \gets 0$ to $p_{end}$}
        \State reliably-send ($i,v_i,p$) 
        \State \textbf{Wait until} $|R_i[p]| \geq n-f$ %\Comment{receiving $n-f$ phase-$p$ messages}
        \State $v_i \gets \frac{1}{2}(\max\{R_i[p]\}+\min\{R_i[p]\})$
    \EndFor
    \State output $v_i$
    \Statex $\slash\slash$ \textit{Background message handler}
    \Upon{receive($j,v_j,p_j$)} 
        \State $R_i[p_j] \gets R_i[p_j] \cup \{v_j\}$
    \EndUpon
    \Statex
    \Statex
\end{multicols}
\end{algorithmic}
\end{algorithm}



%an event is designed to be tagged with a loosely synchronized timestamp, then a node needs to know when a clock synchronization  is achieved. 

Finally, we use a simple approximate consensus (AC) algorithm as shown in Algorithm \ref{alg:AC} to illustrate the expensive storage complexity. AC is a simplification of prior algorithms \cite{AA_Fekete_aoptimal,AA_Dolev_1986,vaidya_PODC12,Tseng_general}. It relies on emulated reliable channels, and is correct given $n \geq 2f+1$. It executes $p_{end}$ phases. At all time, it maintains a state $v_i$, which is set to its input $x_i$ at initialization. In each phase, it reliably sends its state $v_i$ and phase index $p$ using an RMTP protocol. Then it waits until it receive at least $n-f$ phase-$p$ states. We use $|R|$ to present the size of set $R$. Finally, node $i$ updates its state by taking an average of the maximum and minimum values of the received phase-$p$ states, $R_i[p]$. 

While AC is simple, a (slow) node could potentially requires a large $R_i$. In the worst case, consider a node $i$ that is slow at processing data. Suppose all the other nodes have already proceeded to phase $p_{end}$ while $i$ is still at phase $0$. Then to ensure correctness, node $i$ needs to store all the other nodes' states from phase $0$ to phase $p_{end}$, and (slowly) process them one phase by one phase. Compared to our algorithms, AC needs to store $O(np_{end})$ more data. This indeed is a common issue for the algorithms relying on the reliable channels.


~

Without loss of generality, we can scale the inputs to $[0,1]$ as long as they are bounded by scaling $\epsilon$ down by the same factor. Therefore, we make the following assumption:

\begin{assumption}[Bounded Inputs]
    \label{as:bounded-input} 
    For each node $i$, its input $x_i$ satisfies $x_i\in [0,1]$.
\end{assumption}


\input{crash}

\subsection{Approximate consensus in abstract MAC layer model}

\lewis{Yes, please add $v_{min}, v_{max}$. We will mention that each variable is modified at different places in the algorithm description.}

\begin{algorithm}
\caption{MAC-AC Algorithm: Steps at each node $i$}
\label{alg:MAC-AC}
\begin{algorithmic}[1]
\item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
\item[] $p_i$ \Comment{phase, initialized to $0$}
\item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
\item[] $p_{\new}$ \Comment{temporary index for the next phase}
\item[] $v_{\new}$ \Comment{temporary value for the next phase}
\item[] $v_{min}, v_{max}$ \Comment{minimum and maximum heard states, initialized to $v_i$}

\item[] \hrulefill    
\begin{multicols}{2}
    \For{$p_i \gets 0$ to $p_{end}$}
        \State \texttt{lock}()
        \State $v_{min} \gets v_i;~~~ v_{max} \gets v_i$
        \State $p_{\new} \gets p_i$
        \State \texttt{unlock}()
        \State \texttt{mac-broadcast}($v_i, p_i$) \label{line:MAC-AC-mac-broadcast}
        % This guarantees that if a node receives a message, it has to process it before updating
        %\State \textbf{wait until} there is no pending message
        
        %\Statex \hspace{20pt} to be processed by the background handler
        \If{$p_{\new} = p_i$} \label{line:MAC-AC-wait}
            \State \qinzi{\texttt{lock()} we also want to lock $v_{max}, v_{min}$?}
            \State $v_i \gets \frac{1}{2}(v_{max} + v_{min})$ 
            \State $p_i \gets p_i + 1$ \Comment{Move to phase $p_i+1$}
            \label{line:MAC-AC-move}
            \State \qinzi{\texttt{unlock()}}
        \Else 
            \State \texttt{lock()}
            \State $v_i \gets v_{\new}$
            \State $p_i \gets p_{\new}$ \label{line:MAC-AC-jump}
            \State \texttt{unlock()}
        \EndIf
    \EndFor
    \State output $v_i$
    
    \item[] $\slash\slash$ \textit{Background message handler}
    \Upon{receive($v_j,p_j$)} 
        \If{$p_j > p_{\new}$}
            \State \texttt{lock}()
            \State $p_\new \gets p_j$
            \State $v_\new \gets v_j$ \Comment{Jump to phase $p_j$} 
            %after line 6 is executed}
            \State \texttt{unlock}()
        \ElsIf{$p_j = p_{\new} $}
            \If{$v_j > v_{max}$}
                \State $v_{max} \gets v_j$
            \EndIf 
            \If{$v_j < v_{min}$}
                \State $v_{min} \gets v_j$
            \EndIf 
        \EndIf
    \EndUpon
    \Statex
    \Statex
    \Statex
\end{multicols}
\end{algorithmic}
\end{algorithm}


Let $i$ be a node and $p$ be a phase. In this algorithm, the definition of a phase is more straightforward: phase $p$ of node $i$ starts at line 2 and ends at line 16. We then make the following definitions. First, we define $v_i[p]$ as the phase-$p$ state of $i$ and $\perp$ if node $i$ skipped phase $p$ or crashed before phase $p$. Next, we define $V[p]$ as the multiset of phase-$p$ states, excluding $\perp$. For simplicity, define $min_p=\min V[p], max_p=\max V[p]$. We also define $R_i[p]$ as the set of all the messages (of form $(v',p')$) received by node $i$ in phase $p$ (i.e., all messages received starting from line 2 until right before executing line \ref{line:MAC-AC-wait}).  Next, we denote $i_p$ as the first node that updated to phase $p+1$. \lewis{We might need to define $i_p$ as the first node completing line 6. This is because the first node moves to phase $p+1$ might NOT be the first node completing line 6...} If multiple nodes update to $p+1$ concurrently, we let $i_p$ be any one of them. Finally, recall that the there are two ways for node $i$ in phase $p$ to proceed to a higher phase:  (i) \textit{jumps} to phase $p'>p$ if it executes line \ref{line:MAC-AC-jump}; and (ii)  \textit{moves} to phase $p+1$ if it executes line \ref{line:MAC-AC-move}. By construction, only one line will be executed.

% Note that for all $i,p$ such that $v(i,p)\neq \perp$, $R(i,p)$ is non-empty. \lewis{Why? They might receive their own message?} Moreover, there exists at most one $(v',p')\in R(i,p)$ such that $p' > p$. \qinzi{so this is incorrect?} \lewis{I guess so, but it really depends only which line of $R$ you're looking at.}

% \qinzi{so even when node $i$ receives a higher-phase message. it must still wait until it receives Ack in order to proceed to a higher phase? \lewis{Correct.} So it's possible that $i$ receives two higher-phase messages (e.g., the first in phase 10, and the second in phase 15, and it updates to phase 15 at the end?} \lewis{Correct.}

\begin{lemma}
\label{lem:MAC-AC-move-nodes}
Let $j$ be a node other than $i_p$ that \textbf{moves} to phase $p+1$. Then we have
\[
v_j[p+1] \in \left[\frac{min_p+v_{i_p}[p]}{2}, \frac{max_p+v_{i_p}[p]}{2}\right].
\]
\end{lemma}

\begin{proof}
% First for simplicity, assume nodes didn't move to phase $p+1$ concurrently. 
%Let $j$ be any node other than $i_p$ that moved to phase $p+1$. 
Suppose at time $T$, node $i_p$ updated to phase $p+1$ and at time $T'<T$, $i_p$ completed $\texttt{mac-broadcasting}$ (line \ref{line:MAC-AC-mac-broadcast}). By the property of the abstract MAC layer, all nodes that had not crashed at time $T'$, including node $j$, must have received message $(v_{i_p}[p],p)$. By definition, $i_p$ is the first node that updated to phase $p+1$, so node $j$ was in phase $\leq p$ at time $T'$. Furthermore, the message processing assumption as specified in Section \ref{s:message-processing} ensure that all messages received by node $j$ at time $T'$ have been processed before executing line \ref{line:MAC-AC-wait}. 
%\lewis{I think we still need to assume that nodes process at a rough speed; otherwise, it's possible that node $j$ got stuck between line 7 and line 8 (say idling for a long time), and during this time, node $i_p$ completed the mac-broadcast... we want to rule out this case.} 
%In conclusion, there exists $p'\leq p$ such that $(v_{i_p}[p],p) \in R_j[p']$. 

This holds even for $j$ that moved to phase $p+1$ concurrently with node $i_p$ at time $T$. \lewis{move this sentence outside the proof, and elaborate a bit more.}

% Now note that if $j$ moves to phase $p+1$, then (i) $(v_{i_p}[p],p)\in R_j[p]$ and (ii) for all $(\cdot,p'')\in R_j[p]$, $p''\leq p$. We can prove by contrapositive. First, if message $(v_{i_p}[p],p)$ is received by node $j$ in some phase $p'<p$, then it must perform the jump mechanism and jump to phase $p$. \qinzi{it seems that we don't need (ii)}

Since by assumption, node $j$ moves to phase $p+1$, it must be the case that $(v_{i_p}[p],p)\in R_j[p]$. %We then prove the lemma by contrapositive: If message $(v_{i_p}[p],p)$ is received by node $j$ in some phase $p'<p$, then it must perform the jump mechanism and jump to phase $p$. 
Finally, define $S=\{v:(v,p)\in R_j[p]\}$, i.e., the multiset of phase-$p$ states received by node $j$ in phase $p$. Since node $j$ moved to phase $p+1$ (line \ref{line:MAC-AC-move}), $v_j[p+1]=\frac{1}{2}(\min S+\max S)$. Note that $S\subseteq V[p]$, so $\min V[p]\leq \min S \leq \max S\leq \max V[p]$. Next, $v_{i_p}[p]\in S$, so $\min S \leq v_{i_p}[p] \leq \max S$. In conclusion,
\[
\frac{\min V[p] + v_{i_p}[p]}{2}\leq v_j[p+1] = \frac{\min S+\max S}{2} \leq \frac{v_{i_p}[p] + \max V[p]}{2}.
\]
% Now we relax the assumption of concurrent updates, and assume node $j$ moved to phase $p+1$ concurrently at time $T$.
\end{proof}

\begin{theorem}
For any $p\geq 0$,
\[
\max V[p] - \min V[p] \leq \frac{\max V[0] - \min V[0]}{2^p}.
\]
\end{theorem}

\begin{proof}
Consider any phase $p+1$. Node $j$ with $v_j[p+1]\neq \perp$ must update to phase $p+1$ by either jumping or moving. If it moved to phase $p+1$, then by Lemma \ref{lem:MAC-AC-move-nodes}, 
\[
v_j[p+1] \in \left[\frac{min_p+v_{i_p}[p]}{2}, \frac{max_p+v_{i_p}[p]}{2}\right].
\]
If it jumped to phase $p+1$, then there exists some node $k$ such that $v_j[p+1] = v_k[p+1]$ and node $k$ moved to phase $p+1$. In other words, node $k$ is essentially the source node where $j$ copies its state from. Then $v_k[p+1]$ also satisfies the equation above. In conclusion, this equation holds for any $v_i[p+1]$ for any node $i$. Therefore,
\[
\max V[p+1] - \min V[p+1] \leq \frac{\max V[p] - \min V[p]}{2}.
\]
We then prove the theorem by unrolling this recursive expression.
\end{proof}

In conclusion, Algorithm MAC-AC converges exponentially fast in $O(2^{-p})$ rate.

==> byzantine.tex <==
\section{Byzantine Approximate Consensus}
\label{sec:byz}

We now consider a more adverse scenario with Byzantine faulty nodes that may have an arbitrary behavior. Up to $f$ nodes may have Byzantine behavior (denoted as set $\calB$), and the rest of the nodes (denoted as set $\calH$) are fault-free and always follow the algorithm specification. We present an approximate consensus algorithm, \textit{SmallBAC}, which is correct for $n\geq 5f+1$. Algorithm SmallBAC and Algorithm SmallAC share a similar structure, but SmallBAC has different update rules to cope with Byzantine faults. Plus, nodes do \textit{not} skip phases in SmallBAC. The pseudo-code is presented in Algorithm \ref{alg:BACR}.

Each node starts with phase $0$ and initializes its local state $v_i$ to the given input $x_i$. Then it periodically broadcasts its current local state. For each node in phase $p$, upon receiving $n-f$ states from phase $p$ or higher, it updates its local state to the average of the ($f+1$)-st lowest state and the ($f+1$)-st highest state that have been received so far and then proceeds to phase $p+1$. This update rule ensures that the new state falls in the range of fault-free states despite of the existence of Byzantine messages. Moreover, since at most $f$ nodes are Byzantine faulty, this step is always non-blocking. 
Every node repeats this process until phase $p_{end}$, whose value will be determined later in Equation (\ref{eq:p-end-byz}).

SmallBAC is inspired by the original iterative Byzantine approximate consensus algorithm (BAC) \cite{AA_Dolev_1986}, which update states using states from the same phase (similar to the update rule in Algorithm AC). BAC relies on reliable channels; hence, may also need to store $O(np_{end})$ states. SmallBAC may store and update states using messages from different phases (as shown in the $\textsc{Store}(-)$ function below). These subtle differences allow us to reduce the storage complexity, but make the correctness proof more complicated.

Both BAC and SmallBAC require $n \geq 5f+1$. There exists a Byzantine approximate consensus algorithm \cite{OR_Dolev_2004} that achieves an optimal resilience $n \geq 3f+1$; however, it uses a strong primitive -- reliable broadcast. Section \ref{sec:lower-bound} shows that it is impossible to implement such a strong primitive in lossy networks with a limited storage space.

\begin{algorithm}
\caption{SmallBAC: Steps at each node $i$}
\label{alg:BACR}
\label{alg1}
\begin{algorithmic}[1]
    \State \textbf{Initialization}: $p_i\gets 0$
    \State $v_i\gets x_i$
    \State $R_i\gets$ zero vector of length $n$ 
    \State $R_i[i]\gets 1$
    \State $R_{i,\low}, R_{i,\high}\gets \{\}$
    
    \Repeat 
    \State broadcast($i,v_i,p_i$) periodically
    
    \Upon {receive($j,v_j,p_j$)} \label{line:BACR-atomic1}
        \If {$p_j \geq p_i$ and $R_i[j]=0$}
            \State $R_i[j]\gets 1$
            \State $\textsc{Store}(v_j)$
        \EndIf 
        \Statex \hspace{0.4in}$\slash\slash$ \textit{update with $n-f$ states in phase $p$ or higher}
        \If {$|R_i|\geq n-f$} \label{line:BACR-receive}
            \State $v_i\gets \frac{1}{2}[\max(R_{i,\low})+\min(R_{i,\high})]$
            \State $p_i\gets p_i+1$
            \State \textsc{Reset}()
            \label{line:BACR-atomic2}
        \EndIf
    \EndUpon
    
    \Until {$p_i\geq p_{end}$} \Comment{$p_{end}$ defined in Equation (\ref{eq:p-end-byz})}

    \State output $v_i$

    \vspace{5pt}
    \Function{Reset}{\null}
        \State %Initialize $R_i$:
        $R_i[j]\gets0, \forall j\neq i$ 
        \State $R_{i,\low},R_{i,\high}\gets \{\}$
    \EndFunction
    
    \vspace{5pt}
    \Function{Store}{$v_j$}
        \If {$|R_{i,\low}|\leq f$}
            \State $R_{i,\low}\gets R_{i,\low}\cup \{v_j\}$
        \ElsIf {$|R_{i,\low}|=f+1$ and $v_j < \max(R_{i,\low})$}
            \State replace the maximum element in $R_{i,\low}$ with $v_j$
            % \State $\max(R_{i,\low}) \gets v_j$ 
            % \qinzi{not sure if it's a valid notation of ``replacing the maximum element with $v_j$''} \lewis{Use English will be better.}
        \EndIf
        
        \If {$|R_{i,\high}|\leq f$}
            \State $R_{i,\high}\gets R_{i,\high}\cup \{v_j\}$
        \ElsIf {$|R_{i,\high}| = f+1$ and $v_j>\min(R_{i,\high})$}
            % \State $\min(R_{i,\high}) \gets v_j$
            \State replace the minimum element in $R_{i,\high}$ with $v_j$
        \EndIf 
    \EndFunction
\end{algorithmic}
\end{algorithm}

\paragraph*{Storage Complexity}

In Algorithm SmallBAC, each node $i$ stores the following variables ($1$ integer, $2f+3$ floats, and one $n$-bit bit-vector).
\begin{itemize}
    \item $p_i\in\N$: current phase, implemented as an integer;
    \item $v_i\in\R$: local state, implemented as a float;
    \item $R_i\in\{0,1\}^n$: an $n$-bit bit-vector, where each bit $j$ records whether node $i$ has received a message from node $j$ or not; 
    \item $R_{i,\low}, R_{i,\high}$: lists that store the $f+1$ lowest (highest) received states in phase $p$ or higher. Received states are implemented as floats, and each list has length $f+1$. 
\end{itemize}
Recall that $|R_i|$ denotes the number of ones in $R_i$, whereas $|R_{i,\low}|$ and $|R_{i,\high}|$ denote the cardinality (i.e., the number of elements) of $R_{i,\low}$ and $R_{i,\high}$, respectively.

\subsection*{Correctness of Algorithm SmallBAC}

%\subsection*{SmallBAC: Termination}

\begin{theorem}
    Algorithm SmallBAC satisfies termination.
\end{theorem}

\begin{proof}
    We prove termination by induction on phase $p\geq 0$. Formally, we define the induction statement as: every fault-free nodes proceeds to phase $p$ within finite time. The base case holds because all nodes are initially in phase $0$. Now suppose all fault-free nodes proceed to phase $p$ within finite time. Then after all fault-free nodes are in phase $p$ or higher, by assumption of eventual progress (Assumption \ref{as:eventual-progress}), every fault-free node receive at least $n-f$ states from fault-free nodes in phase $p$ or higher within the time bound $\Delta$. Hence, every fault-free proceed to the next phase according to line \ref{line:BACR-receive} -- \ref{line:BACR-atomic2}, which proves the induction.
\end{proof}

\subsection*{SmallBAC: Validity}

We define $V^{(p)}$ and $W^{(p)}$ in a similar way as we did in the previous section. The difference is that we only consider fault-free nodes.

\begin{definition}
Define $V^{(p)}=\{v_1^p,\ldots,v_{|V^{(p)}|}^p\}$ as the multiset of phase-$p$ states of all \textit{fault-free} nodes $i\in\calH$, ordered chronically. By termination, $|V^{(p)}|=h$ for all $p\geq0$, where $h=|\calH|\geq n-f$.

For $k\in [h]$, define $V_k^{(p)}=\{v_1^p,\ldots,v_k^p\}$, i.e., the first $k$ elements in $V^{(p)}$. If $k=0$, we define $V_0^{(p)}=\varnothing$.

Define $W^{(p)}=\{w_1^p,\ldots,w_h^p\}$ as $V^{(p)}$ ordered by values, i.e., $w_1^p\leq \ldots \leq w_h^p$.

Define $U=\{u_1,\ldots,u_b\}$ as a multiset of \textit{arbitrary} values from Byzantine nodes, where $b=|\calB|\leq f$.
\end{definition}

For convenience of analysis, we assume that at most one event will happen in every time moment $t$. More formally, we assume that each node will not receive two messages at the same time. Moreover, two nodes will not proceed to the next phase at the same time. This assumption is reasonable given that time is continuous; otherwise, it is straightforward to use ID as a tie-breaker. We also assume that SmallBAC starts at time $t_0=0$. These assumptions validates the following definitions.

\begin{definition}
\label{def:k_t}
% \qinzi{Which notation is better $k_{t,p}$ or $k(t,p)$? I personally find the latter clearer especially when $k(t,p)$ is used as a subscript.} \lewis{Yes, let's use the latter.}

For time $t\in\R^{\geq0}$ and phase $p\geq 0$, define $k(t,p)$ as the number of fault-free nodes that are in phase $p$ or higher at time $t$. 

For example, at the beginning when $t_0=0$, $k(0,0)=h$ and $k(0,q)=0$ for all $q>0$ because all nodes are initially in phase $0$.
\end{definition}

\begin{definition}
\label{def:set-T-SmallBAC}
Define $T$ as the set of time moments when some fault-free node updates its phase to phase $p$ such that $1\leq p\leq p_{\mathrm{end}}$. We assume $T$ is sorted in ascending order, i.e., $T=\{t_0=0<t_1<t_2<\ldots\}$.
\end{definition}

\begin{remark}
Observe the following properties of $k(t,p)$ and $T$:
\begin{enumerate}
    \item For fixed $p\geq 0$, $k(t,p)$ is non-decreasing with respect to $t$, i.e., $t_1<t_2$ implies $k(t_1,p)\leq k(t_2,p)$. 
    
    For fixed $t\in \R^{\geq 0}$, $k(t,p)$ is non-increasing with respect to $p$, i.e., $p<q$ implies $k(t,p) \geq k(t,q)$.
    
    % \qinzi{This is true by definition, not sure if I need to explain it in detail.} \lewis{Just say be definition.}
    
    \item By termination, every fault-free node updates to phase $p_{\mathrm{end}}$ within finite time. Therefore, set $T$ is finite.
    
    \item Each node doesn't change its local state until it updates its phase. Therefore, the states of all nodes remain unchanged during the interval $(t_k,t_{k+1})$.
\end{enumerate}
\end{remark}

\begin{lemma} %\lewis{Why is this called weak validity?} \qinzi{because it proves weak validity (not in exact input space but instead in range [0,1])?}\lewis{What do you mean? Eq. (3) proves validity as in Def. 1. Did I miss something?} \qinzi{Ah, no. I thought it was called ``weak validity''.} \lewis{OK. Yeah, it's called validity. Weak validity is another term that applies only to Byzantine exact consensus.}
    \label{lem:BACR-weak-validity}
    For every time moment $t_i\in T$,
    \begin{equation}
        \label{eq:BAC-lem-validity}
       \rho(V_{k(t_i,q)}^{(q)}) \subseteq \rho(V_{k(t_i,p)}^{(p)}) ,\ \forall 0 \leq p < q.
    \end{equation}
\end{lemma}

Recall that $\rho(V)$ denotes the interval of $V$, i.e., $\rho(V) = [\min(V),\max(V)]$. %The proof is presented in Appendix \ref{app:lem:BACR-weak-validity}.

\begin{proof}
    We prove the lemma by induction on $t_i$. 
    
    In the base case, $t_0=0$. Recall that $k(0,0)=h$, and $k(0,q)=0$ for every $q>0$. Therefore, $V_{k(0,0)}^{(0)}=V^{(0)}$ and $V_{k(0,q)}^{(q)}=\varnothing$, and thus Equation (\ref{eq:BAC-lem-validity}) is trivially true.
    
    In the induction case, assume Equation (\ref{eq:BAC-lem-validity}) holds for $t_i$ for all $i\in [k]$, and we want to prove for $t_{k+1}$. Consider the fault-free node, say node $i^*$, that updates at time $t_{k+1}$. Assume it updates from phase $p^*$ to $p^*+1$, and denote its state in phase $p^*+1$ as $v^*$. Note that
    \begin{equation*}
    \begin{array}{ll}
        V_{k(t_{k+1},q)}^{(q)} = V_{k(t_k,q)}^{(q)},\ \forall q\neq p^*+1; \\
        V_{k(t_{k+1},p^*)}^{(p*)} = V_{k(t_k,p*)}^{(p)}\cup \{v^*\}.
    \end{array}
    \end{equation*}
    Hence, to prove Equation (\ref{eq:BAC-lem-validity}), it suffices to show that $v^*\in \rho(V_{k(t_k,p*)}^{(p)})$. Then Equation (\ref{eq:BAC-lem-validity}) follows directly from the induction assumption.
    
    Recall that in phase $i^*$, $R_{\low}$ and $R_{\high}$ of node $i^*$ stores $f+1$ lowest (highest) among the $n-f$ received states respectively. In addition, these $n-f$ received states are either from Byzantine states or from nodes in phase $p^*$ or higher. Denote $I$ as the interval of all fault-free received states. Then the $f+1$-st lowest and the $f+1$-st highest received states (i.e., $\max(R_{\low})$ and $\min(R_{\high})$) are both in $I$ because at most $f$ received states are Byzantine. Therefore, $v^*=\frac{1}{2}[\max(R_{\low})+\min(R_{\high})]$ is also in $I$.
    
    Finally, since $I$ is the interval of states in phase $p^*$ or higher, induction assumption implies that
    \begin{equation*}
        I \subseteq \bigcup_{q\geq p^*} \rho(V_{k(t_k,q)}^{(q)}) \subseteq \rho(V_{k(t_k,p^*)}^{(p^*)})
    \end{equation*}
    because $\rho(V_{k(t_k,q)}^{(q)}) \subseteq \rho(V_{k(t_k,p^*)}^{(p^*)})$ for all $q\geq p^*$.
\end{proof}

Lemma \ref{lem:BACR-weak-validity} proves validity of Algorithm SmallBAC by substituting $t=t_{|T|}$, $p=0$ and $q=p_{\pend}$ into Equation (\ref{eq:BAC-lem-validity}) because $k(t_{|T|},0)=k(t_{|T|},p_{\pend})=h$ and thus
\begin{equation*}
    V^{(p_{\pend})} = V_{k(t_{|T|},p_{\pend})}^{(p_{\pend})} \subseteq \rho(V^{(0)}),
\end{equation*}
where $\rho(V^{(0)})$ is the range of the input space.

\subsection*{SmallBAC: $\epsilon$-agreement}

\begin{definition}
Define $a_k^p$ and $A_k^p$ recursively as:
\[
a_{k+1}^p = (a_k^p+w_{1}^p)/2, \enspace A_{k+1}^p = (A_k^p+w_{h}^p)/2,
\]
with initial values $a_0^p=A_0^p=w_{2f+1}^p$.
\end{definition}

Notice two useful properties. First, since $w_1^p\leq w_{2f+1}^p\leq w_h^p$, we have
\[
w_1^p\leq a_k^p \leq w_{2f+1}^p\leq A_k^p \leq w_h^p.
\]
Moreover, using geometric series, their explicit formula are:
\begin{align*}
a_k^p 
&= 2^{-k}w_{2f+1}^p+\sum_{i=1}^k 2^{-i}w_1^p \\
&= w_1^p+2^{-k}(w_{2f+1}^p-w_1^p).
\end{align*}
Similarly, $A_k^p=w_h^p+2^{-k}(w_{2f+1}^p-w_h^p)$.

\paragraph*{Technical Difficulty}
In addition to the effect of Byzantine values, we also need to consider the case when a node uses values from different phases when updating. This is more complicated to analyze than the case of Algorithm SmallAC, since in our prior analysis, a node simply jumps to a future state that trivially satisfies the induction statement. Also, we cannot apply the prior proofs for the traditional Byzantine fault model with  reliable channel (e.g., \cite{AA_Dolev_1986,LocalWait,AA_nancy,OR_Dolev_2004}) either. This is again because that any pair of fault-free nodes may not receive a common message.

We need to prove that the new state of a node falls in a smaller interval as it updates to a higher phase. In the base case, each node in phase $p$ receives non-Byzantine messages from a fixed multiset $V^{(p)}$. By the classical common value analysis \cite{AA_nancy,AA_Dolev_1986}, all nodes in the base case must receive at least one common message from a fault-free node. 

In the more general inductive step, this technique no longer works, because each node can also receive messages from higher phase(s). We need to show that \textit{all fault-free nodes} must share some common information. It turns out that each pair of fault-free nodes may \textit{not} receive a common value. Instead, we show that each fault-free node must receive at least one non-Byzantine message in a \textit{common multiset} (a generalized concept of common value). We then bound the range of this common multiset using $a_k^p$ and $A_k^p$, which allows us to derive the desired convergence rate.
The detailed proof is presented below, and the illustration of common multiset is presented in Figure \ref{fig:BACR-agreement}. 
% Moreover, we have to use double induction, instead of a single induction in prior works \cite{AA_nancy,AA_Dolev_1986}, to make the proof concise.

\begin{figure*}[!ht]
    
    \begin{subfigure}{.32\textwidth}
    \centering
    %\includesvg[width=0.8\linewidth]{./new-fig/test_data_time.svg}
    \includegraphics[width=.95\linewidth]{./new-fig/loss_rate_time.pdf}
	\caption{Convergence time}
    \label{fig-sub:loss-rate-time}
    \end{subfigure}%
    \begin{subfigure}{.32\textwidth}
    \centering
    %\includesvg[width=0.9\linewidth]{./new-fig/test_data_rx.svg}
    \includegraphics[width=.95\linewidth]{./new-fig/loss_rate_rx.pdf}
	\caption{Amount of data received}
    \label{fig-sub:loss-rate-rx}
    \end{subfigure}%
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{./new-fig/loss_rate_tx.pdf}
    %\includesvg[width=0.9\linewidth]{./new-fig/test_data_tx.svg}
	\caption{Amount of data sent}
    \label{fig-sub:loss-rate-tx}
    \end{subfigure}%

	\caption{Impact of Message Loss Rate}
	\label{fig:loss-rate} 
	\vspace{-10pt}
\end{figure*}

\begin{figure*}[!ht]
    
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{./new-fig/scalability_time.pdf}
	\caption{Convergence time}
    \label{fig-sub:scalability-time}
    \end{subfigure}%
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{./new-fig/scalability_rx.pdf}
	\caption{Amount of data received}
    \label{fig-sub:scalability-rx}
    \end{subfigure}%
    \begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{./new-fig/scalability_tx.pdf}
	\caption{Amount of data sent}
    \label{fig-sub:small-tx}
    \end{subfigure}%

    \caption{Scalability}
	\label{fig:scalability} 
	\vspace{-10pt}
\end{figure*}

\begin{lemma}
\label{lem:BACR-agreement}
Suppose $n\geq 5f+1$. Then for every $k\in [h]$,
\begin{equation}
    \label{eq:BAC-thm-agreement}
    v_k^{p+1}\in[a_k^p, A_k^p],\ \forall p\geq 0.
\end{equation}
\end{lemma}

The full proof is presented in Appendix \ref{app:lem:BACR-agreement}.



\begin{theorem}
    Algorithm SmallBAC satisfies $\epsilon$-agreement under $n\geq 5f+1$.
\end{theorem}

\begin{proof}
    Lemma \ref{lem:BACR-agreement} implies that $\rho(V^{(p+1)})\subseteq [a_n^p,A_n^p]$, and recall that
    \begin{align*}
        a_n^p=w_{1}^p+2^{-n}(w_{2f+1}^p-w_1^p), \\ A_n^p=w_{h}^p+2^{-n}(w_{2f+1}^p-w_h^p).
    \end{align*}
    and  $w_1^p=\min V^{(p)}$ and $w_h^p=\max V^{(p)}$.
    Hence, $A_n^p-a_n^p$ gives an upper bound of convergence rate, which is $\delta(V^{(p+1)})\leq (1-2^{-n})\delta(V^{(p)})$.
    
    In conclusion,  SmallBAC satisfies $\epsilon$-agreement at $p_{\mathrm{end}}$, where
    \begin{equation}
        \label{eq:p-end-byz}
        p_{\mathrm{end}} = \frac{\log\epsilon}{\log(1-2^{-n})},
    \end{equation}
    because for all $p\geq p_{\mathrm{end}}$,
    $\delta(V^{(p)})\leq (1-2^{-n})^{p_{\pend}}\leq \epsilon$.
\end{proof}

% \qinzi{An interesting (possibly) worst case example}

% Next, we present a simple example to show that the worst case convergence rate is at least $(1-2^{-2f})$, i.e., $\delta(V^{(p+1)})\geq (1-2^{-2f})\delta(V^{(p)})$.

% Suppose there are $n=5f+1$ nodes. $2f+1$ fault-free nodes have inputs $0$, $2f$ fault-free nodes have inputs $1$, and the rest $f$ are Byzantine faulty.
% \[
% \text{phase $0$:}\ \underbrace{{\color{blue}0,0,\ldots,0},{\color{red}0}}_{2f+1}, \underbrace{{\color{red}1,1,\ldots,1}}_{2f}, \underbrace{b_1,\ldots,b_f}_{f}.
% \]

% The $2f$ nodes with state $1$ and one node with state $0$ (red) experience high receiving delay. They will receive $2f+1$ $0$'s, $f$ $1$'s and $f$ Byzantine states after other nodes proceed to phase $1$. All Byzantine values are negative so that they will update to $\textsc{Reduce}(f,R_i)=0$.

% The other $2f$ nodes with state $0$ (blue) are fast and have no message delay. The first node receives $2f$ $1$'s, $f+1$ $0$'s, and $f$ Byzantine values greater than $1$, and updates to $1/2$. Similarly, the second node receives $2f$ $1$'s, $f$ $0$'s, one $1/2$ and $f$ Byzantine values greater than $1$, and updates to $3/4$.
% In conclusion, the configuration in phase $1$ is as follows.
% \[
% \text{phase $1$:}\ \underbrace{0,0,\ldots,0}_{2f+1}, \underbrace{1/2,3/4,\ldots,1-2^{-2f}}_{2f}, \underbrace{b_1,\ldots,b_f}_{f}.
% \]
% We can repeat this process in each phase, and the range decreases only by $(1-2^{-2f})$.
% Hence, this shows that in the worst case, $p_{\mathrm{end}}$ is exponential with $f$.

% \qinzi{Counter-example of BACR for $n=5f$}

% Consider there are $2f$ fault-free nodes with inputs $0$ and another $2f$ fault-free nodes with inputs $1$. The rest $f$ are Byzantine faulty. In first phase, all $0$ nodes receive $2f$ $0$'s, $f$ $1$'s and $f$ $-1$'s from Byzantine nodes. Then they will update to $0$. Similarly, all $1$ nodes receive $2f$ $1$'s, $f$ $0$'s and $f$ $2$'s from Byzantine nodes, and they will update to $1$. Hence, the configuration won't change in each phase.

==> conclusion.tex <==
\section{Conclusion}

In conclusion, we studied fault-tolerant approximate consensus algorithms in lossy networks with small devices. We proposed algorithm SmallAC that solves crash-tolerant approximate consensus and algorithm SmallBAC that solves Byzantine approximate consensus.
We built a custom simulator on top of Mininet to evaluate more practical properties such as convergence time, network bandwidth, scalability, etc. We also presented two lower bounds for the family of iterative algorithms. 
 There are many interesting open problems left in this domain. We list two here: 

\begin{itemize}
    %\item Under what condition, can an algorithm be adapted with the ``jump-\&-copy'' technique so that the adapted version works in the lossy network with limited storage?
    
    \item What is the optimal convergence rate of the approximate consensus algorithms in our model?
    
    \item What is the lower bound on the storage size for a more general algorithm?
\end{itemize}


==> crash.tex <==
%\section{Crash-Tolerant Approximate Consensus}
%\label{sec:crash}

\subsection{AC in Lossy Link Model}

\qinzi{I modified algorithm description of Loss-AC, please check, thanks!}

This section considers crash faults in lossy network. 
We present a simple algorithm, \textit{Algorithm Loss-AC}, that achieves approximate consensus for $n\geq 2f+1$. Our algorithm is inspired by Algorithm AC. Both adopt a similar  iterative algorithm structure. We have two innovations to cope with lossy networks and reduce storage complexity: periodic broadcast and ``jump'' to a future phase when receiving a state with a larger phase index. The pseudo-code of Loss-AC is presented in Algorithm \ref{alg:Loss-AC} below.


Each node $i$ initializes its local state $v_i$ to a given input $x_i$. To avoid the reliance on reliable channel, each node periodically broadcasts its current $v_i$ every $t$ units of time (line \ref{line:Loss-AC-broadcast} in Algorithm \ref{alg:Loss-AC}). Assumption \ref{as:eventual-progress} ensures that other fault-free nodes will receive at least one state at some point in the $\Delta$-time interval, e.g., $m_3$ in Figure \ref{fig:CR-lossy}. Note that our algorithm does not use $\Delta$, as it is an unknown parameter. We only use it for our convergence analysis. 

One potential drawback, compared to Algorithm AC, is that Loss-AC might waste network bandwidth by periodically broadcast messages. For example, TCP retransmits lost messages only when necessary, whereas Loss-AC proactively broadcasts states even if a received might have already received a same state. 
\qinzi{Do we still have this evaluation section? If not, we don't need this paragraph?}
Later in Section \ref{s:eval}, we will see that the network consumption is on par with Algorithm AC; hence, we do not believe this is an issue. Plus, connected things in real-world usually broadcast  heartbeat/control messages periodically. Loss-AC can piggyback its message over the these messages. 

To reduce storage complexity, we do not store all the states received. Instead, each node $i$ only stores the maximum and minimum received states, denoted by $v_{max}, v_{min}$. \qinzi{Besides, it also stores an $n$-bit counter $R_i$, which is initialized to the unit vector $\mathbf{e}_i$ (i.e., $R_i[i]=1$ and $R_i[j]=0$ for all $j\neq i$). $R_i[j]$ indicates whether $i$ receives a message from $j$. Every time when $i$ receives from an unheard node $j$ (i.e., $R_i[j]=0$), it updates $R_i[j]$ to $1$ (line \ref{line:Loss-AC-counter-update}). We use the notation $|R_i|$ for the number of $1$'s in $R_i$.} 

Consequently, each node $i$ updates state $v_i$ using a different approach from AC. Concretely, for each node $i$ in phase $p$, there are two ways to proceed to a higher phase: 
\begin{enumerate}
    \item (line \ref{line:Loss-AC-jump'} -- \ref{line:Loss-AC-jump}): upon receiving a message from phase $q > p$, node $i$ directly copies the received state and ``jumps'' to phase $q$; or
    
    \item (line \ref{line:Loss-AC-move'} -- \ref{line:Loss-AC-move}): upon receiving $n-f$ phase-$p$ states, node $i$ updates its state and proceeds to phase $p+1$. In this case, we say node $i$ ``moves'' to phase $p+1$. This part is similar to prior work (e.g., Algorithm \ref{alg:AC}). The key difference is that we only store a maximum and minimum of received phase-$p$ states.
\end{enumerate}
Every fault-free node repeats this process until it proceeds to the termination phase $p_{end}$, which will be defined later in Equation (\ref{eq:p-end-crash}). 

\qinzi{Do we keep this paragraph?} With our simple techniques, the convergence seems obvious, since intuitively, state values from ``future phases'' should be ``closer'' to the final output. However, the formal proof is not as straightforward. As we will see next, prior proof techniques (e.g., \cite{AA_nancy,welch_book,LocalWait,AA_Dolev_1986,OR_Dolev_2004}) do not apply, and we have to devise a new proof approach. \qinzi{If my proof is correct, it's no longer that different from the classical arguments...}

\begin{algorithm}
\caption{Loss-AC Algorithm: Steps at each node $i$}
\label{alg:Loss-AC}
\begin{algorithmic}[1]
\item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
\item[] $p_i$ \Comment{phase, initialized to $0$}
\item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
\item[] $p_{next}$ \Comment{temporary index for the next phase, initialized to $p_i$}
\item[] $v_{next}$ \Comment{temporary value for the next phase, initialized to $v_i$}
\item[] $v_{min}, v_{max}$ \Comment{minimum and maximum heard states, initialized to $v_i$}
\item[] $R_i$  \Comment{counter, \qinzi{initialized to unit vector $\mathbf{e}_i$}}
\item[] \hrulefill    
\begin{multicols}{2}
    \Repeat 
        \State broadcast($i,v_i,p_i$) periodically
        \label{line:Loss-AC-broadcast}
        \Upon{$p_{next} > p_i$}
            \State \texttt{lock}()
            \State $v_i \gets v_{next}$
            \State $p_i \gets p_{next}$
            \State $v_{min}, v_{max} \gets v_i$
            \State $R_i \gets \e_i$
            \State \texttt{unlock}()
        \EndUpon
    \Until {$p_i\geq p_{end}$ }
    % \Comment{$p_{end}$ defined in Equation (\ref{eq:p-end-crash})}
    
    \State output $v_i$

    % \Function{Reset}{\null}
    %     \State $R_i[i]\gets 1$, and $R_i[j]\gets 0,\forall j\neq i$
    %     \State $v_{min}, v_{max}\gets v_i$ 
    % \EndFunction
    
    % \vspace{5pt}
    % \Function{Store}{$v_j$}
    %     \If {$v_j < v_{min}$}
    %         \State $v_{min} \gets v_j$
    %     \ElsIf {$v_j > v_{max}$}
    %         \State $v_{max} \gets v_j$
    %     \EndIf
    % \EndFunction
    
    \columnbreak
    
    \item[] $\slash\slash$ \textit{Background ``sequential'' message handler}
    \Upon{receive($j,v_j,p_j$)} \label{line:ACR-start}
        % \Statex \hspace{0.35in} $\slash\slash$ \textit{copy state and jump to future phase}
        \If {$p_j > p_i$} \label{line:Loss-AC-jump'}
            \State \texttt{lock}()
            \State $v_{next}\gets v_j$
            \State $p_{next}\gets p_j$ \Comment{Jump}
            \label{line:Loss-AC-jump}
            \State \texttt{unlock()}
        \ElsIf {$p_j = p_i$ and $R_i[j]=0$} \label{line:ACR-phase-p}
            \State $R_i[j]\gets 1$
            \label{line:Loss-AC-counter-update}
            \If {$v_j < v_{min}$}
                \State $v_{min} \gets v_j$
            \ElsIf {$v_j > v_{max}$}
                \State $v_{max} \gets v_j$
            \EndIf
            \If{$|R_i| \geq n-f$} 
            \label{line:Loss-AC-move'}
                \State $v_{next}\gets \frac{1}{2}(v_{min}+v_{max})$
                \State $p_{next}\gets p_i+1$ \Comment{Move}
                \label{line:Loss-AC-move}
            \EndIf
        \EndIf 
    \EndUpon
    
\end{multicols}    
\end{algorithmic}
\end{algorithm}


% \paragraph*{Storage Complexity}

% In Algorithm Loss-AC, each node $i$ only stores the following variables at all time: $1$ integer, $3$ floats, and an $n$-bit bit-vector (or an array of $n$ Booleans):

% \begin{itemize}
%     \item $p_i\in\N$: phase index, implemented as an integer;
%     \item $v_i\in\R$: local state\footnote{In later proof, we will show that the range of local states strictly shrinks, and consequently $v_i\in[0,1]$ in all phases.}, implemented as a float;
%     \item $v_{\min,i},v_{\max,i}\in \R$: the minimum and maximum received states, both implemented as floats;
%     \item $R_i\in\{0,1\}^n$: an $n$-bit bit vector, where each bit $j$ records whether node $i$ has received a phase-$p$ state from node $j$ or not.
% \end{itemize}
% For brevity, denote the number of ones in vector $R_i$ by $|R_i|$. 

Algorithm AC and other algorithms that assume reliable channels need to store at least $O(n)$ floats (state values) at all time, and may need to store $O(np_{end})$ floats in the worst case, as analyzed in Section \ref{s:prior}. Loss-AC saves storage space by at least a constant factor ($O(n)$ bits vs. $O(n)$ floats), and $O(p_{end})$ in the extreme case.

% \lewis{Correct. We don't need it.}
% \qinzi{We don't need Atomic Execution any more? 
% \paragraph*{Atomic Execution}
% Recall that we assume that a crash-prone node can crash at any point of time and does not remember the last line executed after recovery. Therefore, we require that in our algorithm, some consecutive steps of the algorithms (a block of codes) are executed \textit{atomically}, i.e., these steps are either all executed or none is executed. 

% In Algorithm ACR, the message handler (line \ref{line:ACR-start} -- \ref{line:ACR-end}) is an atomic block. By Assumption \ref{as:eventual-progress}, within $\Delta$ time, between any pair of crash-prone nodes, the sender's message is received and successfully processed. In other words, in every $\Delta$-time interval, at least one message from every crash-prone sender is processed by the message handler (this atomic block of codes) at the receiver.}

% \paragraph*{Key differences}
% Our algorithm has two differences from prior solutions in the traditional crash fault model  \cite{LocalWait,AA_Dolev_1986,OR_Dolev_2004}(e.g., Algorithm \ref{alg:AC}): 

% \begin{itemize}
%     \item (i) each node can ``jump'' to a future phase (line \ref{line:ACR-jump}); and
    
%     \item (ii) each node stores only a max phase-$p$ state and a min phase-$p$ state (line \ref{line:ACR-add-state}).
    
%     %directly \qinzi{aggregates} received value to its local state (line \ref{line:ACR-add-state}). \qinzi{no longer has this feature}
% \end{itemize}

% As mentioned in Section \ref{s:prior}, prior algorithms process messages in the increasing order of phases. Our design reduces the space usage, since Loss-AC does not need to store all the messages received.

%Each node $i$ stores the received value by adding to its local state. Once it receives at least $n-f$ messages in the same phase, it updates to the next phase by dividing its local state by $|R_i|$, which is equivalent to averaging all received value in this phase. During the process, if node $i$ receives a message from a higher phase $p$, then it directly ``jumps'' to phase $p$ with the same state.

\subsection*{Correctness of Algorithm Loss-AC}

Algorithm Loss-AC satisfies termination because each node must receive either $n-f$ messages in the same phase or a message with a higher phase owing to the assumption of \textit{Eventual Progress} (Assumption \ref{as:eventual-progress}). Validity is also straightforward because of our updating rules. Hence, we focus on the $\epsilon$-agreement in our proof.

\paragraph*{Technical Challenge}
$\epsilon$-agreement is tricky to prove, since prior proofs (e.g., \cite{AA_nancy,welch_book,LocalWait,AA_Dolev_1986,OR_Dolev_2004}) rely on the fact that a pair of nodes receive at least \textit{one common value }for each phase (via a typical quorum intersection argument). Since nodes may not receive any message from some phase in our scenario, we need to develop a new proof.
%The key challenge is to device the setup so that we can use induction to derive a bound on the convergence rate. Roughly speaking, the convergence rate identifies the ratio that the range of fault-free nodes decreases in each phase. %The way we define and use $V^{(p)}$ introduced later is different from prior proofs \cite{LocalWait,AA_Dolev_1986,OR_Dolev_2004}.
%Our induction-based proof is useful for handling the case when nodes may not receive common values.
\qinzi{This is true for Byzantine case, but for crash case, common value still works. so maybe we don't need this paragraph any more?} 


\paragraph*{Convergence Proof} \lewis{Given the new algorithm structure, it's not that clear what ``in phase $p$'' means. You might want to define it first.}
Let $i$ be a node and $p$ be a phase. 
\qinzi{First, we formalize the definition of phase $p$ of node $i$. Suppose node $i$ updates $p_i$ to $p$ in line 6, then phase $p$ of node $i$ starts right after line 9 is executed. Phase $p$ ends after the condition $p_{next}>p_i$ is triggered (i.e., right before line 4 is executed).} 
Note that $v_i$ remains fixed during phase $p$, and we define it as the phase-$p$ state of node $i$, denoted by $v_i[p]$. For completeness, $v_i[p]=\perp$ if node $i$ skipped phase $p$ or crashed before phase $p$. Next, we define $V[p]$ as the multiset of phase-$p$ states of all nodes, excluding $\perp$. For simplicity, define $min_p=\min V[p], max_p=\max V[p]$, and $median_p=\median V[p]$.

% \begin{definition}
%     Let $S$ be a finite multiset. Define the \textit{cardinality} $|S|$ as number of elements in $S$ counting multiplicity, the \textit{range} of $S$ as $\delta(S)=\max(S)-\min(S)$, and the \textit{interval} of $S$ as $\rho(S)=[\min(S),\max(S)]$.
% \end{definition}

% \begin{definition}
%     \label{def:ACR-Vp}
%     Define $V^{(p)}$ as a multiset of phase-$p$ states of all nodes. For a crash-faulty node which crashed before phase $p$, its phase-$p$ state is empty and hence is excluded in $V^{(p)}$. Denote $n_p=|V^{(p)}|$.
    
%     % Since the algorithm satisfies termination condition, for every $0\leq p\leq p_{\mathrm{end}}$, $V^{(p)}$ always contains phase-$p$ states of all crash-prone nodes, and thus $n_p\geq h$. Recall that $h = |\calH|$, the size of the set of crash-prone nodes.
    
%     For convenience, we order $V^{(p)}$ \textit{chronologically}. In other words, $V^{(p)}=\{v_1^p,\ldots,v_{n_p}^p\}$, where $v_k^p$ is the phase-$p$ state of the $k$-th node that proceeded to phase $p$. We also define $V^{(p)}_k=\{v_i^p:i\in[k]\}$, i.e., the first $k$ elements in $V^{(p)}$.
    
%     Define $W^{(p)}$ as $V^{(p)}$ sorted in ascending order of values, i.e., $W^{(p)}=\{w_1^p,\ldots, w_{n_p}^p\}$ such that $w_1^p\leq \ldots \leq w_{n_p}^p$.
% \end{definition}

% We then prove the following key lemma to identify the convergence rate. The base case is similar to the ``common value'' technique in \cite{LocalWait,AA_Dolev_1986,OR_Dolev_2004}. The difference lies in the inductive step where we need to consider nodes that skip phases due to the ``jump'' updating rule. Later in Section \ref{sec:byz}, we generalize the technique to handle Byzantine nodes, where the proof naturally becomes more complicated.

\begin{lemma}
\label{lem:Loss-AC-move-nodes}
Assume $n\geq 2f+1$. If node $j$ \textbf{moves} to phase $p+1$, then
\[
v_j[p+1] \in \left[ \frac{min_p + median_p}{2}, \frac{max_p + median_p}{2}  \right].
\]
\end{lemma}

\begin{proof}
The proof is similar to the classical common value argument. Assume node $j$ moved to phase $p+1$ from phase $p$, and let $R_j$ be the indicator vector at the end of phase $p$ (before line 4). \lewis{Is this the line the end of phase $p$? } \qinzi{see the formal definition of phase} We define $S=\{v_i~\text{as received at line 12}:~R_j[i]=1\}$, i.e., the multiset of phase-$p$ states received by node $j$ in phase $p$. Then by line \ref{line:Loss-AC-move'} in Algorithm \ref{alg:Loss-AC}, $|S| = sum(R_j) \geq n-f$. Since we assume $n\geq 2f+1$, $n-f > n/2$. Therefore, $|S|\geq \frac{1}{2}|V[p]|$, and there must exist $v,v'\in S$ such that $v\geq \median V[p]$ and $v'\leq \median V[p]$. Moreover, $v,v'\in S$ implies that
\[
\median V[p] \leq v\leq \max S \quad \textit{and} \quad \min S \leq v' \leq \median V[p].
\]
Furthermore, $S\subseteq V[p]$ implies that $\min V[p] \leq \min S \leq \max S\leq \max V[p]$.

Finally, note that the new state of $j$ is $v_j[p+1] = \frac{1}{2}(\min S+\max S)$. Hence,
\[
\frac{\min V[p] + \median V[p]}{2} \leq v_j[p+1] = \frac{\min S + \max S}{2} \leq \frac{\median V[p] + \max V[p]}{2}.
\]
\end{proof}

\begin{theorem}
Assume $n\geq 2f+1$. For any $p\geq 0$,
\[
\max V[p] - \min V[p] \leq \frac{\max V[0] - \min V[0]}{2^p}.
\]
\end{theorem}

\begin{proof}
Consider any phase $p+1$. Node $j$ with $v_j[p+1]\neq \perp$ must update to phase $p+1$ by either jumping or moving. If it moved to phase $p+1$, then by Lemma \ref{lem:Loss-AC-move-nodes}, 
\[
v_j[p+1] \in \left[\frac{min_p+median_p}{2}, \frac{max_p+median_p}{2}\right].
\]
If it jumped to phase $p+1$, then there exists some node $k$ such that $v_j[p+1] = v_k[p+1]$ and node $k$ moved to phase $p+1$. In other words, node $k$ is essentially the source node where $j$ copies its state from. Then $v_k[p+1]$ also satisfies the equation above. In conclusion, this equation holds for any $v_i[p+1]$ for any node $i$. Therefore,
\[
\max V[p+1] - \min V[p+1] \leq \frac{\max V[p] - \min V[p]}{2}.
\]
We then prove the theorem by unrolling this recursive expression.
\end{proof}

\qinzi{Given Lemma 3 is true, Theorem 4 and Theorem 7 just follow the same logic (and are basically the same). }

\begin{theorem}
    Algorithm Loss-AC satisfies $\epsilon$-agreement after phase $p_{\mathrm{end}}$, where
    \begin{equation}
        \label{eq:p-end-crash}
        p_{\mathrm{end}} = \log_{\frac{1}{2}}(\epsilon) = -\frac{\log(\epsilon)}{\log(2)}.
    \end{equation}
\end{theorem}

% === add if there are extra space ===

% There are alternative updating rules for Algorithm ACR if we enlarge the persistent storage. One alternative rule is that upon receiving $n-f$ phase-$p$ states, each node updates its new state to $\frac{\max+\min}{2}$, where $\max,\min$ denote the maximum and minimum received phase-$p$ states. This method, often denoted as the $reduce$() function in previous works \cite{}, gives a faster convergence rate. Since all nodes are guaranteed to receive at least one common state, the range of new states are guaranteed to decrease by at least $\frac{1}{2}$, i.e., $\delta(V(p+1))\leq \frac{1}{2}\delta(V(p))$. However, this requires a larger persistent storage as each node stores three values: (1) phase number; (2) minimum received state; and (3) maximum received state, as well as the $n$-bit counter. In the next section, we will adapt the $reduce()$ function in the new algorithm to achieve a faster convergence rate.

==> firstMover.tex <==
\begin{algorithm*}
\caption{MAC-DoubleFirstMover Algorithm: Steps at each node $i$ with input $v_i$}
\label{alg:MAC-FirstMover}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:} /* These variables can be accessed by any thread at node $i$. */]{}

\item[] $coin_i$ \Comment{value, initialized to $\perp$}
% \vspace{-5pt}
% \item[] \hrulefill    

\item[{\bf Fixed parameter:}]{ $\tilde n$} \Comment{an estimation of $n$}
% \vspace{-5pt}
\item[] \hrulefill    
\vspace{-15pt}
\begin{multicols}{2}
    \State $k \gets 0$
    \While{$coin_i = \perp$}
        \If{a local random number $< \frac{2^k}{2\tilde n}$}
            \State $\texttt{mac-broadcast}(\texttt{COIN}, v_i)$
        \Else
            \State $\texttt{mac-broadcast}(\texttt{DUMMY})$
        \EndIf
        \State $k \gets k+1$
    \EndWhile
    \State \textbf{return} $coin_i$
    \columnbreak
    \item[$\slash\slash$ \textit{Background message handler}]
    \Upon{receive($\texttt{COIN}, v$)} 
        %\State $\texttt{mac-broadcast}(\texttt{COIN}, v)$
        \State $coin_i \gets v$
    \EndUpon
    \item[]
    \Upon{receive($\texttt{DUMMY}$)} 
        \State \textbf{do} nothing
    \EndUpon
\end{multicols}
\vspace{-10pt}
\end{algorithmic}
\end{algorithm*}

==> lower_bound.tex <==
\section{Lower Bounds}

\label{sec:lower-bound}

We present two lower bounds for the following family of algorithms. Our approximate algorithms belong to this family of algorithms. It is a generalization of iterative algorithm in the traditional fault model with reliable channel, e.g., \cite{AA_Dolev_1986,AA_nancy,LocalWait,OR_Dolev_2004}. These two lower bounds show that SmallAC has an asymptotically optimal space complexity and SmallBAC has an optimal resilience within the family of the iterative algorithms introduced next.

\subsection{Iterative Algorithms}

%\qinzi{Reviewer 1: For example, when you say ``each bit in C reflects whether it has received and processed a message from a certain node or not, i.e., the bit is 1 if it is received, and 0 otherwise;'' - doesn't it immediately imply that a process can only remember messages received from |C| processes? Further, assuming that ``every node uses the same counter and predicate'' should mean this should the same set of processes everywhere?} \lewis{OK. Not hard to address. You can leave editing it to me. Please go over them carefully to see if we use crash-recovery anywhere. Or if we just assume typical crash.} \qinzi{I don't think we assumed crash-recovery. I think the only underlying assumption is that every node must periodically broadcast its current state because message might be lost during communication. And this assumption only requires lossy link + typical crash/Byzantine.} \lewis{OK. Great. Thanks for checking.} \qinzi{No problem!}

Each node $i$ is initially in phase $0$ with local state equal to its input $x_i$. It propagates information by broadcasting its current state tagged with the current phase index periodically, and proceeds to higher phases until a termination phase $p_{end}$. Each node $i$ performs the following two steps in phase $p$:

\begin{itemize}
    
    \item \textit{Receive}: keep receiving messages until a certain condition/predicate is met. Denote by $R_i$ the multiset of messages that node $i$ had received and decided to store; and
    
    \item \textit{Update}: update state using a transition function $Z_i$ which takes $R_i$ to a real number $Z_i(R_i)\in \rho(R_i)$.
\end{itemize}

\paragraph*{Space Constraint}
Recall that with an unbounded persistent storage, one can simulate the reliable channel model using an RMTP protocol \cite{Reliable-transmission_JACM1994}, and we can apply prior algorithms \cite{OR_Dolev_2004,LocalWait,AA_Dolev_1986}. Therefore, we have a practical constraint on the storage size, which is bounded by a constant $c$. That is, the storage space is pre-allocated before the execution of the algorithm with size $c$. 



\subsection{Space Complexity: Lower Bound on Number of Bits}

We first show the number of bits of the required storage complexity. Recall that the family of algorithms we consider must store a state value $v$ and a phase index. Hence, we are interested in the \textit{additional} number of bits that need to be stored. We prove the following theorem in Appendix \ref{app:space}.


\begin{theorem}
\label{thm:lower-bound-bit}
    For all the correct iterative approximate consensus algorithms using an $r$-bit counter as the predicate, $r \geq f+2$.
\end{theorem}

In other words, the size of the persistent storage $c$ has to be large enough to store a state, a phase index, and $(f+2)$ bits. This theorem shows that our ACR algorithm is asymptotically optimal.



\subsection{Lower Bound on Number of Nodes}

Abraham et al. \cite{OR_Dolev_2004} presented an optimal algorithm in the traditional Byzantine model with reliable channel. One key insight is to use reliable broadcast (RB) primitive \cite{Bracha:1987} to make sure faulty nodes cannot equivocate, i.e., sending mismatching messages to different nodes. We prove that $n \geq 5f+1$ is necessary in our model by (i) first arguing that each node cannot use RB to periodically transmit its state if $c$ is bounded and allocated a priori; and (ii) constructing a scenario that equivocating faulty nodes have the ability to force two groups of crash-prone nodes to output values that violate the $\epsilon$-agreement if $n \leq 5f$. We prove the following theorem in Appendix \ref{app:resilience}.



\begin{theorem}
    \label{thm:resilience}
    In lossy networks with Byzantine faults and nodes with limited storage space, $n=5f+1$ is a necessary condition to solve approximate consensus.
\end{theorem}



==> mac-approximate.tex <==
\section{Anonymous Storage-Efficient Approximate Consensus}
\label{s:approximate}

We first discuss the problem definition, followed by our wait-free  algorithms. The first algorithm MAC-AC requires higher space complexity, but the proof is simpler and achieves exponential convergence. The second algorithm MAC-AC2 requires the knowledge of the upper bound on the network size, and has worse convergence. However, it requires only two values and one Boolean, which we conjecture to achieve optimal storage complexity. 

We are not aware of any prior  approximate consensus algorithms that aim to reduce storage complexity. For example, most algorithms, e.g.,  \cite{AA_Dolev_1986,LocalWait,vaidya_PODC12}, in the standard message-passing model store the messages from at least a quorum of nodes, making the space complexity linear with the network size $n$. On the other hand, the approach of stacking prior algorithms  \cite{ApproximateConsensus_Moran1995,welch_book} on top of MAC-SC also require linear space complexity due to the usage of the store-collect object. 

%\subsection{Approximate Consensus Problem}

\begin{definition}[Approximate Consensus \cite{AA_Dolev_1986}]
    A correct approximate consensus algorithm  needs to satisfy: (i) \textit{Termination}: Each fault-free node decides an output value within a finite amount of time; (ii) \textit{Validity}: The outputs are within the range of the inputs; and (iii) \textit{$\epsilon$-agreement}: The outputs of all fault-free nodes are within $\epsilon$.
    
    %     \begin{itemize}
    %     \item[(i)] \textit{Termination}: Each fault-free node decides an output value within a finite amount of time;
        
    %     \item[(ii)] \textit{Validity}: The outputs are within the range of the inputs; and 
        
    %     \item[(iii)] \textit{$\epsilon$-agreement}: The outputs of all fault-free nodes are within $\epsilon$.
    % \end{itemize}
\end{definition}

Following the literature \cite{LocalWait,AA_nancy,welch_book}, we assume that the range of initial inputs of all nodes is bounded. This is  typical in many connected devices applications that are sensing nearby environments. For example, inputs could be temperature, air pollution level, target location, etc. 
Without loss of generality, we scale the inputs to $[0,1]$. %as long as they are bounded by scaling $\epsilon$ down by the same factor. %Therefore, we make the following assumption:

% \begin{assumption}[Bounded Inputs]
%     \label{as:bounded-input} 
%     For each node $i$, its input $x_i$ satisfies $x_i\in [0,1]$.
% \end{assumption}


\subsection{Algorithm MAC-AC and Correctness Proof}

We next present Algorithm MAC-AC. The pseudo-code is presented in Algorithm \ref{alg:MAC-AC}. The algorithm adopts the iterative structure from prior works, e.g.,  \cite{AA_Dolev_1986,LocalWait,vaidya_PODC12}. Nodes proceed in phases, and their state is attached with a phase index. 
% Each node has a main thread and a background message handler side thread. The main thread proceeds sequentially so that a line starts to execute only when the previous line completes and there is no pending messages in the message handler. The message handler triggers whenever node $i$ receives a message in the abstract MAC layer. Due to our message processing model described in Section \ref{sec:message-processing}, the handler is pended when the main thread is locked and resumes when unlocked.
%Each node $i$ is given an input $x_i \in [0, 1]$. Then 
Node $i$ initializes phase index $p_i=0$ and state value $v_i=x_i$, its input in $[0, 1]$. To reduce storage space, each node does not store all the received messages as in prior algorithms, e.g., \cite{AA_Dolev_1986,vaidya_PODC12,LocalWait}. Instead, node $i$ only stores two extra states: the maximum and minimum received states, denoted by $v_{max}$ and $v_{min}$, respectively. These two values are only updated by the message handler. 

One feature of prior algorithms is that nodes always proceed phase by phase. This requires nodes in phase $p$ to store messages from higher phases so that slow nodes could eventually catch up. We introduce a simple ``jump'' technique to avoid such storage of old messages -- upon receiving a state from a higher phase $p$, a node can simply copy the state and ``jump'' to the phase $p$. 
Node $i$ uses $p_{next}$, $v_{next}$, and a Boolean $jump$ to decide how to proceed to a higher phase.

At the beginning of each phase $p_i$, node $i$ resets $v_{min}, v_{max}$. Then it use the abstract MAC layer to broadcast its current phase index and value (line \ref{line:MAC-AC-mac-broadcast}). Meanwhile, the background message handler may receive and process  messages from other nodes. After node $i$ receives the acknowledgement of its $\texttt{mac-broadcast}$ primitive, it concludes the current phase by deciding how to proceed to a higher phase (line 8-13) with the following two approaches:
\begin{enumerate}
    \item (line 8-10): If node $i$ did not receive any message of the form $(v,p_j)$ with $p_j>p_i$, then it updates to phase $p_i+1$ with state $(v_{min}+v_{max})/2$. In this case, we say node $i$ ``\textit{moves}'' to phase $p_i+1$.
    \item (line 11-12): If node $i$ received some message with a higher phase, then it copies the received state and phase. 
    %depending on the order of message handling, it copies the state and phase of a processed message $(v_j,p_j)$ with highest phase. 
    In this case, we say node $i$ ``\textit{jumps}'' to phase $p_j$.
\end{enumerate}
Each node repeats this process until phase $p_{end}$. Observe that messages could arrive and be processed at any point of time. To ensure that $p_i$ and $v_i$ are always in sync, we use locks to protect the reset (line 3 and 4) and update (line 8 to 12) procedures. 

We use a single lock to ensure a block of codes are executed atomically. By assumption, \texttt{mac-broadcast} is not atomic; hence, the message handler could process messages during any point of time between line 5 and line 7. 

%We will prove in Theorem \ref{thm:MAC-AC-converge} that Algorithm MAC-AC converges in exponential rate; hence, $p_{end}$ is of order $O(\log\frac{1}{\epsilon})$ to achieve $\epsilon$-agreement. The correctness of prior algorithms rely on the fact that a pair of nodes receive at least one common value for each phase (via a typical quorum intersection argument). Even though as observed in \cite{AbstractMAC_randomizedConsensus_DISC2018}, a quorum-based approach is not feasible in the abstract MAC layer, we can still rely on the property of \texttt{mac-broadcast} to identify such a common value. 

% \begin{algorithm}
% \caption{MAC-AC Algorithm: Steps at each node $i$}
% \label{alg:MAC-AC}
% \begin{algorithmic}[1]
% \item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
% \item[] $p_i$ \Comment{phase, initialized to $0$}
% \item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
% \item[] $p_{\new}$ \Comment{temporary index for the next phase}
% \item[] $v_{\new}$ \Comment{temporary value for the next phase}
% \item[] $v_{min}, v_{max}$ \Comment{minimum and maximum received states, initialized to $v_i$}

% \item[] \hrulefill    
% \begin{multicols}{2}
%     \For{$p_i \gets 0$ to $p_{end}$}
%         \State \texttt{lock}()
%         \State $v_{min} \gets v_i;~~~ v_{max} \gets v_i$
%         \State $p_{\new} \gets p_i$
%         \State \texttt{unlock}()
%         \State \texttt{mac-broadcast}($v_i, p_i$) \label{line:MAC-AC-mac-broadcast}
%         % This guarantees that if a node receives a message, it has to process it before updating
%         %\State \textbf{wait until} there is no pending message
        
%         %\Statex \hspace{20pt} to be processed by the background handler
%         \State \texttt{lock()}
%         \If{$p_{\new} = p_i$} \label{line:MAC-AC-wait}
%             \State $v_i \gets \frac{1}{2}(v_{max} + v_{min})$ 
%             \State $p_i \gets p_i + 1$ \Comment{Move to phase $p_i+1$}
%             \label{line:MAC-AC-move}
%         \Else 
%             \State $v_i \gets v_{\new}$
%             \State $p_i \gets p_{\new}$ \Comment{Jump to phase $p_j$}  \label{line:MAC-AC-jump}
%         \EndIf
%         \State \texttt{unlock()}
%     \EndFor
%     \State output $v_i$
    
%     \columnbreak
    
%     \item[] $\slash\slash$ \textit{Background message handler}
%     \Upon{receive($v_j,p_j$)} 
%         %\State \texttt{lock()}
%         \If{$p_j > p_{\new}$}
%             \State $p_\new \gets p_j$
%             \State $v_\new \gets v_j$ 
%             % \Comment{Jump to phase $p_j$} 
%             %after line 6 is executed}
%         \ElsIf{$p_j = p_{\new} $}
%             \If{$v_j > v_{max}$}
%                 \State $v_{max} \gets v_j$
%             \EndIf 
%             \If{$v_j < v_{min}$}
%                 \State $v_{min} \gets v_j$
%             \EndIf 
%         \EndIf
%         %\State \texttt{unlock}()
%     \EndUpon
%     \Statex
%     \Statex
%     \Statex
% \end{multicols}
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{MAC-AC: Steps at each node $i$ with input $x_i$}
\label{alg:MAC-AC}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
\item[] $p_i$ \Comment{phase, initialized to $0$}
\item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
\item[] $jump$ \Comment{Boolean, initialized to $false$}
\item[] $v_{min}, v_{max}$ \Comment{minimum and maximum received states, initialized to $v_i$}

\item[] \hrulefill    
\begin{multicols}{2}
    \For{$p_i \gets 0$ to $p_{end}$}
        \State \texttt{lock}()
        \State $v_{min} \gets v_i;~~~ v_{max} \gets v_i$
        \State $jump \gets false$
        \State \texttt{unlock}()
        \State \texttt{mac-broadcast}($v_i, p_i$) \label{line:MAC-AC-mac-broadcast}
        \State \texttt{lock()}
        \If{$jump = false$} \label{line:MAC-AC-wait}
            \State $v_i \gets \frac{1}{2}(v_{max} + v_{min})$ 
            \State $p_i \gets p_i + 1$ \Comment{``Move'' to  $p_i$}
            \label{line:MAC-AC-move}
        \Else 
            \State \textbf{go to} line 3 in phase $p_i$ \Comment{``Jump'' to $p_i$}
        \EndIf
        \State \texttt{unlock()}
    \EndFor
    \State output $v_i$
    
    \columnbreak
    
    \item[$\slash\slash$ \textit{Background message handler}] 
    \Upon{receive($v,p$)} 
        \State \texttt{lock()}
        \If{$p > p_i$}
            \State $p_i \gets p$
            \State $v_i \gets v$ 
            \State $jump \gets true$
        \ElsIf{$p = p_i $}
            \If{$v > v_{max}$}
                \State $v_{max} \gets v$
            \EndIf 
            \If{$v < v_{min}$}
                \State $v_{min} \gets v$
            \EndIf 
        \EndIf
        \State \texttt{unlock}()
    \EndUpon
    \Statex
    \Statex
    \Statex
\end{multicols}
\vspace{-35pt}
\end{algorithmic}
\end{algorithm}

%\paragraph{Correctness Proof}

\noindent\textbf{Correctness Proof}~Validity and termination are obvious, since we consider only crash faults. We focus on the convergence proof below. 
Consider node $i$ at phase $p$. First, we formalize the definition of phase $p$. In each iteration of the for-loop, phase $p$ of node $i$ starts at line 2 and ends at line 6.  %(Observe that the value of $v_i$ remains fixed during this period, and we define it as the phase-$p$ state of $i$, denoted by $v_i[p]$.) \qinzi{$v_i$ can change when it jumps multiple times. maybe change to: 
Although the value of $v_i$ may change during this period, we define the phase-$p$ state of $i$ as $v_i$ \underline{at the beginning of phase $p$}, denoted by $v_i[p]$. %}
For completeness, we define $v_i[p]=\perp$ if node $i$ skips phase $p$ (by jumping to a higher phase) or crashes before phase $p$. 
In other words, node $i$ broadcasts $(v_i[p], p)$ using the abstract MAC layer at line 6; and the MAC layer ensures that every node that has not crashed will receive $v_i[p]$ when line 6 completes, even if the broadcaster crashes afterwards. This implies the following remark:
\begin{remark}
\label{rmk:MAC-AC2}
Every received and processed message is of form $(v_j[p_j],p_j)$ for some node $j$. %That is, $j$'s phase-$p$ state. 
\end{remark}
Next, we define $V[p]$ as the multiset of phase-$p$ states of all nodes, excluding $\perp$. For brevity, we define $min_p=\min V[p], max_p=\max V[p]$. Finally, we denote $i_p$ as the first node that completes line 6 in phase $p$. Since it is the first node, its phase index does \textit{not} change during line 2 and line 6. If multiple nodes complete line 6 concurrently, we let $i_p$ be any one of them. Due to the property of \texttt{mac-broadcast}, $v_{i_p}[p]$  is the ``common value'' received by fault-free nodes that we need to prove convergence. We then prove a key lemma.

\begin{lemma}
\label{lem:MAC-AC-move-nodes}
Let $j$ be a node other than $i_p$ that \textbf{moves} to phase $p+1$. Then we have
\[
v_j[p+1] \in \left[\frac{min_p+v_{i_p}[p]}{2}, \frac{max_p+v_{i_p}[p]}{2}\right].
\]
\end{lemma}

\begin{proof}
% Define $R_j[p]$ as the multiset of all phase-$p$ states  ``received and \textit{processed}'' by the message handler of node $j$ in phase $p$. %(i.e., $v'$ in the message tuple $(v',p)$)
Define $R_j[p]$ as the multiset of all states in the tuple $(v,p)$ ``{received and \textit{processed}}'' by $j$'s message handler in phase $p$.
Due to our message processing model described in Section \ref{sec:message-processing}, the message handler only processes messages when the main thread is not locked, i.e., after line 5 ends and before line 7 starts. By Remark \ref{remark1}, there is no pending message to be processed in the background handler when line 7 starts. Moreover, the handler does not process any message when the main thread is locked, i.e., during line 7 to 13. Therefore, by Remark \ref{rmk:MAC-AC2}, $R_j[p]$ is effectively the multiset of all phase-$p$ states received and processed during the execution of line 5 to 7. Consequently, at line $9$, $v_{max}=\max R_j[p]$ and $v_{min} = \min R_j[p]$;
and $v_j[p+1] = \frac{1}{2}(\min R_j[p]+\max R_j[p])$.

Suppose $i_p$ completed $\texttt{mac-broadcast}$ (line \ref{line:MAC-AC-mac-broadcast}) at time $T$. By the property of the abstract MAC layer, node $j$ has received message $(v_{i_p}[p],p)$ by time $T$. By definition of $i_p$, node $j$ has \textit{not} completed line 6 by time $T$, so it is in phase at most $p$; and the message processing assumption (Remark \ref{remark1}) ensures that all the messages received by node $j$ by time $T$ will be processed before executing line 7. Therefore, $v_{i_p}[p]\in R_j[p']$ for some $p'\leq p$. Since by assumption, node $j$ \textit{moves} to phase $p+1$, it must be the case that $v_{i_p}[p]\in R_j[p]$.
%\lewis{I think we still need to assume that nodes process at a rough speed; otherwise, it's possible that node $j$ got stuck between line 7 and line 8 (say idling for a long time), and during this time, node $i_p$ completed the mac-broadcast... we want to rule out this case.} 
%In conclusion, there exists $p'\leq p$ such that $(v_{i_p}[p],p) \in R_j[p']$. 


% Now note that if $j$ moves to phase $p+1$, then (i) $(v_{i_p}[p],p)\in R_j[p]$ and (ii) for all $(\cdot,p'')\in R_j[p]$, $p''\leq p$. We can prove by contrapositive. First, if message $(v_{i_p}[p],p)$ is received by node $j$ in some phase $p'<p$, then it must perform the jump mechanism and jump to phase $p$. \qinzi{it seems that we don't need (ii)}


Finally, by definition,  $R_j[p]\subseteq V[p]$, so $\min V[p]\leq \min R_j[p] \leq \max R_j[p]\leq \max V[p]$. Moreover, $v_{i_p}[p]\in R_j[p]$, so $\min R_j[p] \leq v_{i_p}[p] \leq \max R_j[p]$. In conclusion,
\[
\frac{\min V[p] + v_{i_p}[p]}{2}\leq v_j[p+1] = \frac{\min R_j[p]+\max R_j[p]}{2} \leq \frac{v_{i_p}[p] + \max V[p]}{2}.
\]
% Now we relax the assumption of concurrent updates, and assume node $j$ moved to phase $p+1$ concurrently at time $T$.
\end{proof}

With some standard arithmetic manipulation and Lemma \ref{lem:MAC-AC-move-nodes}, we can obtain the following theorems, which prove the exponential convergence. (Full proof in Appendix \ref{app:MAC-AC-agrement}.)

\begin{theorem}
\label{thm:MAC-AC-agreement}
For any $p\geq 0$,
\[
\max V[p] - \min V[p] \leq \frac{\max V[0] - \min V[0]}{2^p}.
\]
\end{theorem}

\begin{theorem}
\label{thm:MAC-AC-converge}
Algorithm MAC-AC achieves $\epsilon$-agreement for any $p_{end} \geq \log_2(\frac{1}{\epsilon})$.
\end{theorem}

\subsection{Further Reducing Storage Complexity}

Next we present a simple algorithm, MAC-AC2, in Algorithm \ref{alg:MAC-AC2}, which further reduces storage complexity, assuming the knowledge of an upper bound on the network size. Each node $i$ only keeps three values: state $v_i$, phase $p_i$, and Boolean $jump$. Upon receiving $(v,p)$ from a higher phase $p>p_i$, $i$ jumps to phase $p$ and copies state $v$; and upon receiving $(v,p)$ with  $p=p_i$, it updates its new state to the average of its current state and the received state. 

\begin{algorithm}
\caption{MAC-AC2: Steps at each node $i$ with input $x_i$}
\label{alg:MAC-AC2}
\begin{algorithmic}[1]
\footnotesize
\item[{\bf Local Variables:} /* These variables can be accessed and modified by any thread at node $i$. */]{}
	
\item[] $p_i$ \Comment{phase, initialized to $0$}
\item[] $v_i$ \Comment{state, initialized to $x_i$, the input at node $i$}
\item[] $jump$ \Comment{Boolean, initialized to $false$}
% \item[] $c_i$ \Comment{counter, initialized to $1$}

\item[] \hrulefill
\begin{multicols}{2}
    \For{$p_i \gets 0$ to $p_{end}$}
        \State $jump\gets false$
        \State \texttt{mac-broadcast}($v_i, p_i$) 
        % \State \texttt{lock}()
        \If{$jump = false$}
            \State $p_i\gets p_i+1$ \Comment{``Move'' to $p_i$}
        \Else 
            \State \textbf{go to} line 2 in phase $p_i$ \Comment{``Jump'' to $p_i$}
        \EndIf
        % \State \texttt{unlock}() \qinzi{do we need this lock for this kind of 1 line processing?}
    \EndFor
    \State output $v_i$
    
    \columnbreak
    
    \item[$\slash\slash$ \textit{Background message handler}]
    \Upon{receive($v,p$)}
        \If {$p > p_i$}
            \State $p_i\gets p$
            \State $v_i \gets v$
            \State $jump \gets true$
        \ElsIf {$p = p_i$}
            \State $v_i\gets (v_i+v)/2$
            %\State $jump \gets false$
        \EndIf
    \EndUpon
\end{multicols}
\vspace{-10pt}
\end{algorithmic}
\end{algorithm}

%It turns out that we can further reduce the storage space of Algorithm \ref{alg:MAC-AC} by removing all local variables except $p_i,v_i$. We present the pseudo-code of the new algorithm as Algorithm \ref{alg:MAC-AC2} in Appendix \ref{app:MAC-AC2}. In the new algorithm. we removed the jumping mechanism, and each node $i$ always moves to phase $p_i+1$ in each iteration. Also, when node $i$ receives a message $(v,p)$ with $p\geq p_i$, it updates its state to $(v_i+v)/2$.

This algorithm does not need a lock but requires the knowledge of an upper bound on $n$ to determine $p_{end}$.  Moreover, the convergence rate in the worst case could be as slow as $(1-2^{-n})$. However, we believe that its simplicity makes it appropriate for many small connected devices. 

%\paragraph{Convergence Proof} 
\noindent\textbf{Convergence Proof}~ 
The intuition is straightforward. When a node moves to the next phase, its state is a weighted average of all  received (and processed) states from the same or higher phase. Therefore, the range of all states should shrink strictly. However, the proof requires a  finer-grained setup and more involved arithmetic to obtain the bound. %Without the jumping mechanism, node $i$ might receive messages from higher phase at an early state (when $i$ is in a relatively low phase). However, the messages from a higher phase becomes less effective, in terms of shrinking ranges, compared to the case when $i$ receives more message of the same phase. In the worst case, there is one single node $s$ that proceeds to a high phase $p$, and all other nodes, being slow, receive states from $s$ when they are in phase $0$. \qinzi{do we keep this paragraph?}


We first make the following definitions. Phase $p$ of node $i$ starts at line 2 in Algorithm \ref{alg:MAC-AC2} and ends when line 4 starts. We define the phase-$p$ state of node $i$ as $v_i$ at the beginning of phase $p$, denoted by $v_i[p]$. For completeness, $v_i[p]=\perp$ if $i$ crashes before phase $p$. 
% In other words, node $i$ broadcasts $(v_i[p], p)$ using the abstract MAC layer at the beginning of phase $p$ (line 2); and the MAC layer ensures that every fault-free node will receive $v_i[p]$ when line 2 completes, even if the broadcaster crashes afterwards. This implies the following useful remark:
% \begin{remark}
% \label{rmk:MAC-AC2}
% Every received and processed message is of form $(v_j[p_j],p_j)$ for some node $j$. That is, $j$'s phase-$p$ state. 
% \end{remark}
Next, we define $V[p]$ as the multiset of all phase-$p$ states excluding $\perp$,  and $i_p$ as the \underline{first} node that completes line 2 in phase $p$. %\qinzi{starts line 3 in phase $p$.}
In the following discussion, we use $r$ for the subscripts of messages, and $i, j$ for nodes. 

\begin{theorem}
\label{thm:mac-ac2}
If node $j$ \textbf{moves} to phase $p+1$, then
\[
v_j[p+1] \in \left[ \min V[p] + \frac{v_{i_p}[p]-\min V[p]}{2^{n}}, \max V[p] - \frac{\max V[p]-v_{i_p}[p]}{2^{n}} \right].
\]
\end{theorem}

The proof is in Appendix \ref{app:thm:mac-ac2}. 
Following the same proof of Theorem \ref{thm:MAC-AC-agreement}, we can prove the convergence rate using Theorem \ref{thm:mac-ac2} in the theorem below, which allows us to derive $p_{end}$. 

\begin{theorem}
\label{thm:MAC-AC2-converge}
For any $p\geq 0$,
$\max V[p] - \min V[p] \leq (\max V[0] - \min V[0])(1-2^{-n})^p.$ 
%In particular, if we assume $V[0]=[0,1]$, then Algorithm MAC-AC2 satisfies $\epsilon$-agreement for any $p_{end}$ such that
% \[
% p_{end} \geq \log_{1-2^{-n}}(\epsilon).
% \]
\end{theorem}

%\paragraph{Discussion} We conjecture that MAC-AC2 achieves the optimal storage complexity for achieving approximate consensus. Intuitively, phase is used for determining the termination condition. Suppose nodes do not store messages that they cannot process currently (e.g., due to mismatching phases). Then we believe that the jump mechanism is necessary for nodes to learn states from a higher phase. In this case, the Boolean variable is used to distinguish between moving and jumping so that nodes can keep track of the current phase accurately. 
